The TeV Sun Rises: Discovery of Gamma rays from the Quiescent Sun with HAWC

We report the first detection of a TeV gamma-ray flux from the solar disk (6.3$\sigma$), based on 6.1 years of data from the High Altitude Water Cherenkov (HAWC) observatory. The 0.5--2.6 TeV spectrum is well fit by a power law, dN/dE = $A (E/1 \text{ TeV})^{-\gamma}$, with $A = (1.6 \pm 0.3) \times 10^{-12}$ TeV$^{-1}$ cm$^{-2}$ s$^{-1}$ and $\gamma = -3.62 \pm 0.14$. The flux shows a strong indication of anticorrelation with solar activity. These results extend the bright, hard GeV emission from the disk observed with Fermi-LAT, seemingly due to hadronic Galactic cosmic rays showering on nuclei in the solar atmosphere. However, current theoretical models are unable to explain the details of how solar magnetic fields shape these interactions. HAWC's TeV detection thus deepens the mysteries of the solar-disk emission.

==> Sun_Gamma_HAWC/guest_author.tex <==
\author{J. F. Beacom}
%\email{beacom.7@osu.edu}
%\thanks{\scriptsize \!\!  \href{http://orcid.org/0000-0002-0005-2631}{orcid.org/0000-0002-0005-2631}}
\affiliation{Center for Cosmology and AstroParticle Physics (CCAPP), Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Department of Physics, Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Department of Astronomy, Ohio State University, Columbus, Ohio 43210, USA}

\author{T. Linden}
%\email{linden.70@osu.edu}
%\thanks{\scriptsize \!\!  \href{http://orcid.org/0000-0001-9888-0971}{orcid.org/0000-0001-9888-0971}}
\affiliation{The Oskar Klein Centre, Department of Physics, Stockholm University, AlbaNova, SE-10691 Stockholm, Sweden}

\author{K. C. Y. Ng}
%\email{ chun-yu.ng@weizmann.ac.il}
%\thanks{\scriptsize \!\! \href{http://orcid.org/0000-0001-8016-2170}{orcid.org/0000-0001-8016-2170}}
\affiliation{Department of Physics, The Chinese University of Hong Kong, Sha Tin, Hong Kong, China}

\author{A. H. G. Peter}
%\email{apeter@physics.osu.edu}
%\thanks{ \scriptsize \!\!  \href{http://orcid.org/0000-0002-8040-6785}{orcid.org/0000-0002-8040-6785}}
\affiliation{Center for Cosmology and AstroParticle Physics (CCAPP), Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Department of Physics, Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Department of Astronomy, Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{School of Natural Sciences, Institute for Advanced Study, 1 Einstein Drive, Princeton, NJ 08540}

\author{B. Zhou \vspace{0.5cm}}
%\email{zhou.1877@osu.edu}
%\thanks{\scriptsize \!\!  \href{http://orcid.org/0000-0003-1600-8835}{orcid.org/0000-0003-1600-8835}}
\affiliation{William H. Miller III Department of Physics and Astronomy, Johns Hopkins University, Baltimore, Maryland 21218, USA}





